A Survey on Facial Image Privacy Preservation in Cloud-Based Services

Facial recognition models are increasingly employed by commercial enterprises, government agencies, and cloud service providers for identity verification, consumer services, and surveillance. These models are often trained using vast amounts of facial data processed and stored in cloud-based platforms, raising significant privacy concerns. Users' facial images may be exploited without their consent, leading to potential data breaches and misuse. This survey presents a comprehensive review of current methods aimed at preserving facial image privacy in cloud-based services. We categorize these methods into two primary approaches: image obfuscation-based protection and adversarial perturbation-based protection. We provide an in-depth analysis of both categories, offering qualitative and quantitative comparisons of their effectiveness. Additionally, we highlight unresolved challenges and propose future research directions to improve privacy preservation in cloud computing environments.

==> copy.tex <==
 
\section{State-of-the-art Face Image Protection Approaches}
%{\color{black}To protect private facial information from unauthorized use by commercial deep learning models, various approaches have been proposed in recent years. Existing solutions can be divided into two categories: image obfuscation-based protection methods and adversarial perturbation-based protection methods. This classification is based on how protected images are generated. Image obfuscation techniques entail altering facial features to de-identify the face. This can involve changes in facial characteristics (e.g., gender and makeup) or blending with another image to obtain a new image. With image obfuscation-based protection methods, the resulting image may exhibit visible changes compared to the original faces. Adversarial perturbation-based protection methods add perturbations to the images to make them unlearnable to the attack model, and the perturbations are almost unrecognizable to the human eye. The protected images closely resemble the original private images.}

As the use of cloud-based services for storing and processing facial data continues to expand, the need for robust privacy protection techniques becomes more critical. To address privacy concerns in cloud environments, researchers have developed several state-of-the-art methods to protect facial images from unauthorized exploitation. These techniques are primarily categorized into image obfuscation-based protection methods and adversarial perturbation-based protection methods. Both approaches aim to preserve the utility of facial images while making them unrecognizable or ``unlearnable" to commercial face recognition models used in cloud services.



\subsection{Image Obfuscation-based Protection Methods}

%{\color{black}Based on the location of obfuscation, image obfuscation can be further divided into two categories: specific property obfuscation and whole image obfuscation.}
Image obfuscation methods alter or mask specific characteristics of facial images to make them unrecognizable to facial recognition systems. These methods typically involve modifying identifiable facial features or blending them with other visual elements to prevent accurate face identification.

\subsubsection{Specific properties obfuscation}

{\color{black} %Hu et al. \cite{hu2022protecting} introduced AMT-GAN (adversarial makeup transfer-GAN) using generative adversarial networks (GANs) to create deceptive facial images by transferring makeup from reference images, making it challenging to identify the individual's identity. Due to the application of makeup, the face appears very natural and comfortable. However, this method is primarily designed to protect female images and may not perform well on male images.

Techniques in this category focus on obfuscating certain facial attributes, such as gender, age, or skin texture. For example, AMT-GAN (Adversarial Makeup Transfer-GAN) \cite{hu2022protecting} uses generative adversarial networks (GANs) to apply makeup to a user’s face, making it difficult for face recognition models to accurately identify the individual. This method preserves the overall appearance of the face while making critical identity features difficult to detect. However, this technique is primarily effective for female faces, and adapting it for broader use cases remains a challenge. To address this challenge, Tang et al. \cite{tang2022gender} proposed Gender-AN, a gender-adversarial network that directly confuses gender to protect facial privacy. The face generator in Gender-AN undergoes optimization through a multi-task-based loss function, incorporating attribute manipulation loss, face matcher loss, adversarial loss, and reconstruction loss functions. This optimization approach ensures robust generalization performance while maintaining the natural appearance.
}



%{\color{black}To achieve more fine-grained control over the protected face while preserving the maximum utility, Chen et al. \cite{chen2022mass} introduced MaSS (multi-attribute selective suppression). MaSS enables a meticulous surgical operation on targeted data, allowing the suppression of any selected attribute while leaving the rest unchanged. It employs adversarial games between two sets of networks: one suppresses selected attributes, and the other ensures the retention of the remaining attributes.}

\subsubsection{Whole image obfuscation}


Li et al. \cite{li2021deepblur} proposed DeepBlur, which blurs images in the latent space of a pre-trained generative model capable of creating realistic facial images. The process involves three steps: latent representation search, deep blurring, and image generation. The input face image is transformed into a latent space vector, modified multiple times using a pre-trained model to remove identifying information, and then a realistic face is generated based on the blurred latent space vector model. This approach allows for generating different levels of obfuscation for various applications. However, there is a noticeable visual gap between the generated and original images.

%He et al. \cite{he2024diff} proposed Diff-Privacy, which is a diffusion-based method for facial privacy protection by using advanced diffusion models to anonymize images in cloud-based environments. This approach ensures that facial images are unlearnable by recognition models while maintaining visual quality. The flexibility of this method allows it to meet diverse privacy protection requirements in cloud services.

%In addition to these software-based solutions, Lopez et al. \cite{lopez2024privacy} presented a hardware-level approach to facial privacy protection, using optical encoders to generate face heatmaps that hide identities while preserving the rest of the image for use in cloud-based environments. Such advancements provide another layer of protection, offering a more robust defense against identity-based recognition systems.}

%He et al. \cite{he2024diff} introduced Diff-Privacy, a diffusion-based method for facial privacy protection that leverages advanced diffusion models to anonymize images, particularly in cloud-based environments. Diff-Privacy ensures that facial images become ``unlearnable" by recognition models, while still maintaining a high degree of visual fidelity. This method is particularly flexible, making it well-suited for a wide range of privacy protection needs in cloud services. Its ability to maintain both privacy and visual quality positions it as a robust solution for modern privacy challenges.




{\color{red}He et al. \cite{he2024diff} introduced Diff-Privacy, a more advanced diffusion-based method for anonymizing facial images in cloud-based environments. Diffusion models, originally designed for image generation and restoration, incrementally add noise to an image and then reverse the process to recover or generate a new image. In Diff-Privacy, this diffusion process is employed to introduce noise into facial images in such a way that the images remain unrecognizable by facial recognition systems. Unlike DeepBlur, which directly manipulates the latent space, Diff-Privacy operates at the pixel level to iteratively transform the image. The method maintains high visual fidelity while making the facial data ``unlearnable" by machine learning models. This flexibility allows it to meet varying privacy requirements in cloud-based services, where balancing visual quality and data privacy is critical.

In addition to software-based solutions, Lopez et al. \cite{lopez2024privacy} presented a hardware-level approach to facial privacy protection through the use of optical encoders. Their method generates face heatmaps that obscure the user's identity while preserving other aspects of the image for non-sensitive applications. This hardware-level solution adds another layer of protection, offering a more robust defense against identity-based recognition systems by directly addressing the vulnerabilities that software-based solutions may overlook in cloud environments.

Zhang et al. \cite{zhangtransferable} further addressed the issue of Blind Face Restoration (BFR), where obfuscated facial images could be restored using advanced restoration models. Their transferable adversarial obfuscation method creates obfuscated images that resist restoration attempts by BFR models. This method enhances the generalization of obfuscated faces across various BFR models, ensuring that even if adversaries attempt to retrain restoration models on obfuscated images, the obfuscation remains effective. This technique is particularly valuable in scenarios where attackers have access to BFR systems and aim to reverse facial obfuscation.


}


%Different from AnonymousNet, UP-GAN (utility-preserving GAN) \cite{Hao2019UPGAN} operates solely on the utility information and does not require direct access to the original facial data. Utility information is defined based on facial properties like age, gender, skin tone, pose, and expression. To obscure faces, UP-GAN initially uses an auxiliary system to detect utility information. The fake face is then generated by the UP-GAN model using such information. Since the generated face has the same pose and expression, it can be swapped with the original face using face-swapping algorithms to perform de-identification. UP-GAN preserves a variety of soft biometrics that do not display identity and also achieves k-anonymity.


%To enhance the similarity between the generated and original images, Wu et al. \cite{wu2019PPGAN} introduced PP-GAN (privacy-protective GAN). PP-GAN includes a verificator to eliminate biometric information and a regulator to preserve image utility within the GAN network. It removes biometric details while preserving image quality, including brightness, contrast, and structural similarity. The regulator ensures the consistency between the generated image and the original image by utilizing the pixel-level structure similarity measured through SSIM. However, PP-GAN does not consider k-anonymity privacy protection, leaving the privacy of the entire dataset vulnerable. k-anonymity is a privacy technique in data anonymization. It ensures that individuals in a dataset are not easily distinguishable from at least k-1 other individuals based on certain attributes, aiming to protect individual privacy by making it difficult for adversaries to identify specific people in the dataset.

%Li et al. \cite{AnonymousNet} proposed AnonymousNet as an alternative method that obfuscates facial identities while generating realistic images. This method achieves k-anonymity privacy protection, and it consists of four key steps: facial feature extraction, semantic-based attribute obfuscation, de-identified face generation, and adversarial perturbation. The process begins by utilizing a large number of attribute classifiers to recognize facial attributes. After attribute obfuscation, AnonymousNet utilizes GAN to generate a new facial image with modified attributes. Finally, AnonymousNet adds a kind of antagonistic noise to the generated image to achieve better performance.AnonymousNet can generate realistic images with fake identities and balance privacy and usability in quality and quantity. However, AnonymousNet requires access to the original face data, which may lead to privacy disclosure.


\subsection{Adversarial Perturbation-based Protection Methods}

Adversarial perturbation techniques focus on adding subtle, imperceptible noise to facial images, making them resistant to recognition by machine learning models without significantly altering the visual quality of the image. These perturbations ensure that even if the images are used to train a face recognition model, the model will fail to learn meaningful representations from the data.

{\color{black}We divide the schemes of adversarial perturbation into two categories according to whether requiring auxiliary data or not.}
%Unlike image obfuscation-based methods, which may visibly alter the original images, Adversarial perturbation-based protection methods add perturbations to the images to make them unlearnable to the attack model, and the perturbations are almost unrecognizable to the human eye. The generated protected images are almost the same as the original private image.


\subsubsection{Non-auxiliary data requirement} 

{\color{black} Under such a protection paradigm, the defenders do not rely on any auxiliary dataset to protect the private faces.}
%{\color{black}Cherepanova et al. \cite{cherepanova2021lowkey} proposed LowKey, which protects users from unauthorized surveillance and is made available to the public as a network tool. LowKey alters private faces to create a perturbed version that does not match probe images of the same person. It achieves this by moving the feature space far from the protected image while minimizing perceptual similarity loss. LowKey is the first evasion tool against Amazon Rekognition and the Microsoft Azure Face Recognition APIs. However, it will exhibit visual artifacts and distortions perceptible to the human eye, impacting image quality.
%In addition to generating perturbation for a single image, defenders can generate universal perturbation that can be applied to a specific category, known as class-wise noise. 
Huang et al. \cite{huang2021unlearnable} generated unlearnable examples that contain error-minimizing noises, referred to as EM. It is based on such an intuition: the samples with larger training loss may contain more knowledge to be learned. Generating optimal perturbations that minimize the loss can suppress the informative knowledge of the data, thereby protecting the data from being learned. %Although class-wise noise is much more convenient and efficient, it is more likely to be evaded by adversarial training. To address this challenge,
Further, Fu et al. \cite{fu2021robust} introduced REM (robust error-minimizing noise), which effectively reduces the adversarial training loss and suppresses the learnable knowledge of data in adversarial training.

{\color{black}Zhong et al. \cite{zhong2022opom} presented OPOM (one person one mask) to generate class-wise masks by optimizing each training sample in a direction away from the feature subspace of the protected face image. {\color{black}The feature subspace represents the specific set of features or representations associated with that face, often determined by techniques like class centers, convex hulls, and affine hulls.} OPOM is efficient and suitable for real-time privacy protection applications. However, OPOM may not be effective in scenarios where there are significant differences between the testing images and the training samples, such as larger poses, different illumination, or different occlusions compared to the original protected image.} 

{\color{red}Shamshad et al. \cite{shamshad2024makeup} introduced DFPP, which leverages makeup as an adversarial technique to obfuscate identity in facial images. DFPP employs a deep neural network to transfer makeup features from a reference image to a target image, effectively masking the user's identity while preserving the visual aesthetics. This method is particularly effective in black-box facial recognition environments, where the internal workings of the recognition model are unknown. Although makeup is the medium, the technique generates adversarial perturbations that disrupt the recognition model, making it fall under adversarial perturbation-based methods rather than specific property obfuscation.}

\cite{zhangtransferable}

\begin{figure}[tt]
\vspace{-0.4cm}
	\centering
	\includegraphics[width=9cm]{modelsteal/Figure_1 (1).png}\\
	\caption{Comparison of facial privacy protection performance of EM \cite{huang2021unlearnable}, REM \cite{fu2021robust}, and OPOM \cite{zhong2022opom}.}
    \label{fig:fl}
    \vspace{-0.4cm}
\end{figure}

\begin{figure}[tt]
	\centering
	\includegraphics[width=9cm]{modelsteal/fig.png}\\
	\caption{Comparison of facial privacy protection performance of APF \cite{zhang2020adversarial}, Fawkes \cite{shan2020fawkes}, and TIP-IM \cite{yang2021towards}.}
    \label{fig:2}
    \vspace{-0.6cm}
\end{figure}

\begin{figure*}[tt]
	\centering
	\includegraphics[width=15cm]{c.png}\\
	\caption{Visual comparison results of different facial privacy protection methods.}
    \label{fig:c}
    \vspace{-0.6cm}
\end{figure*}

\iffalse
\begin{figure*}[tt]
	\centering
	%\hspace{-0.8cm}
	\begin{minipage}[t]{3.24in}
		\centering
		\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=3.24in]{b.png}\\
		\centerline{\footnotesize (a) }
	\end{minipage}
	\hspace{-0cm}
	\begin{minipage}[t]{2.61in}
		\centering
		\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=2.61in]{a.png}\\
		\centerline{\footnotesize (b)}
	\end{minipage}
	\hspace{-0cm}
	
	\caption{{\color{black} Visual comparison results of different facial privacy protection methods.}} \label{fig:c}
\end{figure*}
\fi



\subsubsection{Auxiliary data requirement}

{\color{black}In this case, the defender protects private faces with the assistance of an auxiliary dataset.}

%requires an auxiliary dataset to generate the adversarial perturbation.}
%generate the image-independent universal adversarial perturbation or select a target category from it to generate a perturbed image.

{\color{black}
Zhang et al. \cite{zhang2020adversarial} developed APF (adversarial privacy-preserving filter) to protect online shared face images from unauthorized use. APF is an end-cloud collaborated adversarial attack framework and ensures that only users' own devices can access the original images. It involves three key modules: image-specific gradient generation, adversarial gradient transfer, and universal adversarial perturbation enhancement. Image-specific gradient generation extracts gradients on the user end, and adversarial gradient transfer fine-tunes them in the server cloud. The server creates a universal perturbation by maximizing feature distances in an auxiliary dataset. An enhancement module adjusts it to match the image-specific perturbation for better integration.}
{\color{black}In the same period, Shan et al. \cite{shan2020fawkes} proposed Fawkes. In Fawkes, the defender first selects a target category from a publicly auxiliary dataset. Specifically, the authors use a feature extractor to calculate the centroid of the feature space for each candidate class and pick the class whose feature representation centroid is the most dissimilar to the feature representation of all the private images. Then Fawkes randomly selects an image from the target class and optimizes the calculation of the small disturbance of the protected image. In this step, the authors introduced DSSIM (Structural Dissimilarity Index) to ensure that the processed image is visually similar to the original image. However, Fawkes is designed for the white box, requiring access to the feature extractor the user wishes to subvert.}

{\color{black}Unlike Fawkes, Yang et al. \cite{yang2021towards} introduced TIP-IM (targeted identity-protection iterative method) to encrypt private facial images, offering privacy protection against black-box face recognition systems. TIP-IM generates adversarial identity masks and overlays them on facial images, concealing the original identities without compromising visual quality. To create the adversarial identity masks, the authors employ a novel optimization mechanism, using MMD (Max Mean Discrepancy) loss to enhance the visual quality of the crafted adversarial examples. This allows concealing the original images without sacrificing their visual quality, and the generated masks are effective for other black-box models. To control the misclassification results, the authors use greedy insertion to select the optimal victim image from an auxiliary dataset. However, as TIP-IM lacks constraints on visual behavior, except for naturalness defined by MMD, the increase in noise intensity may not guarantee a natural change in pixel information, especially when the de-identification effect dominates naturalness in the face image.}




==> modelsteal/abstract.tex <==
\begin{abstract}
%Facial recognition models have been widely utilized by commercial companies, government organizations, and their contractors for both consumer services and surveillance purposes. These models are trained on user facial images collected from online social networks. However, this raises concerns about the privacy of social media users, as their proprietary images are used to train commercial models without their consent. In recent years, there has been a growing need to prevent unauthorized data leakage and protect the privacy of social media users' facial images.In this article, we conduct a thorough investigation of current methods for protecting the facial privacy of social media users. According to the protected image generation method, we divide these methods into two categories: image obfuscation-based protection methods and adversarial perturbation-based protection methods. We also provide a comprehensive review of each category and provide qualitative and quantitative comparisons to existing methods.Lastly, we identify open issues and potential future research directions to further enhance privacy protection performance.


Facial recognition models are increasingly employed by commercial enterprises, government agencies, and cloud service providers for identity verification, consumer services, and surveillance. These models are often trained using vast amounts of facial data processed and stored in cloud-based platforms, raising significant privacy concerns. Users’ facial images may be exploited without their consent, leading to potential data breaches and misuse. This survey presents a comprehensive review of current methods aimed at preserving facial image privacy in cloud-based services. We categorize these methods into two primary approaches: image obfuscation-based protection and adversarial perturbation-based protection. We provide an in-depth analysis of both categories, offering qualitative and quantitative comparisons of their effectiveness. Additionally, we highlight unresolved challenges and propose future research directions to improve privacy preservation in cloud computing environments.



\end{abstract}
\begin{IEEEkeywords}
Facial image privacy, cloud-based services,  image obfuscation, adversarial perturbation, and facial privacy protection.
\end{IEEEkeywords}



==> modelsteal/comparison.tex <==
\section{Comparison and Evaluation}\label{section:comparision}

\subsection{Qualitative Comparison}
We compare the existing image obfuscation-based protection and adversarial perturbation-based protection methods in Table~\ref{tab:my-table1} and Table~\ref{tab:my-table2}, respectively. 
\begin{itemize}
    \item \emph{API}:
    Commercial facial recognition APIs are widely used by businesses, law enforcement, private entities, and governments. These APIs are typically based on large datasets and are known for their high recognition accuracy. A face privacy protection method that can successfully mislead these APIs is considered to be practical in real-world scenarios. Methods such as AMT-GAN, DeepBlur, and TIP-IM are shown to be effective in protecting against services like Aliyun Face, Microsoft Face, and the Tencent AI Open Platform.
    %AMT-GAN can protect against Aliyun Face service, and DeepBlur can protect against Microsoft Face service. OPOM, and Fawkes can protect against Amazon Rekognition and Microsoft Azure Face, and TIP-IM offers protection against a commercial face search API on the Tencent AI Open Platform.

    \item \emph{Open-set}: 
    In close-set face recognition, the faces used for testing are limited to those identities that are present in the training set, and no individuals outside of the training set will be included. However, in most real-world applications, the face to be recognized is likely to be an identity that is not present in the training set, and in such cases, open-set face recognition is necessary. We can see that only a few methods (e.g., AMT-GAN, Diff-Privacy, and Optics) are effective in open-set face recognition scenarios.

%\item \emph{Black-box}: % 因为在实际情况中，crackers使用的人脸识别模型的具体配置我们是不清楚的，甚至crackers还可能同时使用多种人脸识别模型，所以一个有效的人脸隐私保护方案应该具备在黑盒攻击下依然可用的性能。In real-world scenarios, the precise configuration of the face recognition model employed by attackers is uncertain. Moreover, attackers may use multiple face recognition models at the same time. Therefore, an effective face privacy protection scheme should maintain its effectiveness regardless of the specific model. In black-box cases, the defender has no information about the face recognition model employed by attackers, including the training set, model structure, and parameters. Apart from adversarial perturbation-based protection methods, only AMT-GAN, Gender-AN, DeepBlur, and UP-GAN are shown to be effective in black-box scenarios. %Note that all the adversarial perturbation-based protection methods mentioned above are effective in black-box scenarios.

\item \emph{Real-time capability}:
This metric measures whether the obfuscation method can be applied in real-time. Optics and Diff-Privacy are both capable of real-time application, making them suitable for scenarios such as live video streams. Methods like AMT-GAN and Gender-AN require more processing time, limiting their applicability in real-time systems.

\item \emph{Scalability}:
Scalability measures the method's efficiency when applied to large-scale datasets in cloud environments. Diff-Privacy and DeepBlur show high scalability, as they can be applied efficiently across many images in cloud settings. Optics, being a hardware-based solution, is less scalable due to the need for specific equipment.

\item \emph{Hardware compatibility}:
Methods like Optics require specific hardware for implementation, which may limit their widespread use. Other methods, such as DeepBlur and Diff-Privacy, are software-based, making them more flexible and easier to deploy across various platforms.
 %\item \emph{k-anonymity}: {\color{black}The concept of k-anonymity ensures that for any combination of quasi-identifiers, there must be at least $k$ records in the search results, making it difficult for observers to link records using quasi-identifiers. This measurement of disclosure risk helps to better protect privacy in an anonymized database. We can see that AnonymousNet and UP-GAN can realize the k-anonymity attribute.}
%enhance privacy protection for data sets.

  %\item \emph{Self-supervised}: Supervised learning requires input and output, also known as features and objectives. In contrast, unsupervised learning deals with input data that is not labeled and lacks a definite result. The classification of sample data is unknown, so it is necessary to classify the sample set based on similarities between samples to minimize the gap between intra-class and maximize the gap between inter-class. Apart from DeepBlur, Gener-AN, and AMT-GAN, other image obfuscation-based protection methods use self-supervised learning.

\item \emph{Target-identity}: When creating an adversarial mask, the defender can connect it to a specific target identity for misclassification or any random misclassification identity. It is shown that only Fawkes and TIP-IM belong to target-identity scenarios, where any samples protected by the generated mask will be misclassified into a pre-designed target identity.
%在为受保护图像生成掩码时，是否指定身份类别，使得人脸识别系统错误地将受保护图像识别为这个身份。

 \item \emph{Person-specific}: A person-specific mask is specific to an individual and is similar to class-wise perturbation. Therefore, person-specific mask generation can increase efficiency while maintaining effectiveness. It is shown that EM, REM, and OPOM can support generating person-specific masks.
    
\item \emph{Effective for out-of-distribution data leakage}: In the real world, the attacker can not only access the user's protected images. For example, the attacker can extract the user's unprotected images from the photos shared by his friends. It will incur additional challenges for face privacy protection. Among the existing protection works, it is shown that only EM,  REM, APF, and Fawkes can also maintain the protection ability in such a case.
%Conditional GAN falls under the category of supervised learning, as demonstrated by the usage of this technique in image obfuscation by PP-GAN and UP-GAN. In essence, conditional GAN is a type of supervised learning.

 
\end{itemize}
\begin{table*}[ht]
\centering
\caption{Comparison of the State-of-the-art Image Obfuscation-based Protection Methods.}
\label{tab:my-table1}
\setlength{\tabcolsep}{4.6mm}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Methods   &Whole image obfuscation &API &Open-set &\begin{tabular}[c]{@{}c@{}}Real-time\\capability \end{tabular}& Scalability &\begin{tabular}[c]{@{}c@{}}Hardware\\compatibility \end{tabular}\\ \hline
AMT-GAN \cite{hu2022protecting}     & NO      & YES           & YES  & NO               & Moderate            & NO  \\ \hline
Gender-AN \cite{tang2022gender}    & NO      & Not discussed & NO   & NO                    & Moderate            & NO  \\ \hline
%MaSS   \cite{chen2022mass}       & NO      & Not discussed & NO   & White-box & NO              & YES \\ \hline
DeepBlur  \cite{li2021deepblur}    &YES      & YES           & NO   & YES                    & High             & NO  \\ \hline
%PP-GAN  \cite{wu2019PPGAN}      &YES      & Not discussed & NO   & White-box & NO              & YES \\ \hline

%AnonymousNet \cite{AnonymousNet} &YES      & Not discussed & YES  & White-box & YES             & YES \\ \hline
%UP-GAN \cite{Hao2019UPGAN}    &YES      & Not discussed & YES  & YES                    & YES             & YES \\ \hline
Diff-Privacy \cite{he2024diff}&YES&	YES	&YES&YES&High&NO\\ \hline
Optics \cite{lopez2024privacy}&YES&Not discussed &YES&YES&Low&YES\\\hline

Transferable \cite{zhangtransferable}&YES&YES&YES&YES&High&NO\\\hline

\end{tabular}
%\vspace{-0.4cm}
\end{table*}
\iffalse
\subsubsection{Comparison of adversarial perturbation}
We compare the existing adversarial perturbation-based protection methods in the following five aspects, as shown in Table~\ref{tab:my-table2}. 
\begin{itemize}
    \item \emph{API}:
    LowKey, OPOM, and Fawkes are able to protect against Amazon Rekognition and Microsoft Azure Face, and TIP-IM offers good protection against a commercial face search API on the Tencent AI Open Platform.
  
    \item \emph{Open-set}: 
    Among image obfuscation-based protection methods, only AnonymousNet, UP-GAN, and AMT-GAN are effective in open-set face recognition scenarios.

    \item \emph{Black-box}: 
    Apart from EM and REM, all other adversarial perturbation-based protection methods are shown to be effective in black-box scenarios.
    
    \item \emph{Person-specific}: A person-specific mask is specific to an individual and is similar to class-wise perturbation. Therefore, person-specific mask generation can increase efficiency while maintaining effectiveness.
    
    \item \emph{Effective for out-of-distribution data leakage}: In the real world, the attacker can not only access the user's protected images. For example, the attacker can extract the user's unprotected images from the photos shared by the user's friends. It will incur additional challenges for face privacy protection. Among the existing protection works, it is shown that only EM,  REM, APF, and Fawkes can also maintain the protection ability in such a case.
    %To solve such a challenge, Fawkes proposed a strategy to actively reduce the impact of unprotected image leaks. Studies such as EM, REM, and APF have also examined the effectiveness of this proposed method when only a portion of the image is protected.
    
\end{itemize}
\fi

\subsection{Performance Evaluation}
We compare the protection performance of two types of adversarial perturbation-based protection methods, as the codes for most image obfuscation-based methods are currently unavailable. 

We first evaluate EM, REM, and OPOM, all of which protect social media users' facial privacy without relying on auxiliary data.
The evaluation metrics are protection success rate (PSR) and similarity (SSIM). PSR is defined as the ratio of the number of wrongly recognized images to the total number of images, and SSIM refers to the structural similarity of the two images before and after protection. SSIM is similar to the human visual system and is sensitive to local structural changes. The larger the value, the more similar the protected image is to the original image for the human eye.


In the experiments, we utilized the CASIA-WebFace dataset, which comprises 494,414 images of 10,575 individuals. We randomly selected 50 identities to hide their identities and perturbed 80\% of the images for training the face recognition model, with the remaining 20\% of clean images used for testing. The perturbations were generated separately according to the original source codes. {\color{black}We set the uniform perturbation budget at 0.03.} The face recognition model structure is Inception$\_$Resnet, the training batch size is 64, and the epoch number is 50. The SSIM is calculated for all protected images before and after, with the average value obtained.

The comparison results of these four methods are shown in Fig.~\ref{fig:fl} and Fig.~\ref{fig:c}. %While LowKey boasts a high protection success rate in protection, it results in poor image quality with noticeable distortion patterns to the human eye.} 
It is shown that REM strikes a better balance between protection and image quality. The other two methods exhibit varying degrees of trade-off between protection and image quality. The low success rate of OPOM protection may stem from its limited number of images per identity. %不同方法之间图像质量的差异源于目标函数中对于有界噪声的约束方式不同，同时与是否考虑了感知相似度的损失有关。
%LowKey affects the facial texture, leading to a marked decrease in visual quality. This may be attributed to the use of LPIPS for perceptual similarity calculation. 
As shown in Fig.~\ref{fig:c} (left side), OPOM achieves favorable visual outcomes by using the $L_\infty$ norm to control the maximum value of perturbed elements. % compared to LowKey. 
{\color{black}Regarding noise limitation, EM and REM exhibit comparable image quality.}
%加噪前后对比图的说明：从图中可以看到，LowKey的保护方式改变了人脸的纹理，与其他几种方法相比，视觉质量明显下降，这可能与它使用LPIPS来度量感知相似度有关。OPOM使用L∞范数约束了扰动元素的最大值，获得了比lowkey更好的视觉效果。EM和REM在噪声的限制方法上相似，图片质量从视觉上相差不大。

\begin{table*}[tt]
\centering
\footnotesize
\caption{Comparison of the State-of-the-art Adversarial Perturbation-based Protection Methods.}
\label{tab:my-table2}
\setlength{\tabcolsep}{2.7mm}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Methods &Auxiliary data requirement&API          & Open-set & Target-identity     & Person-specific & \begin{tabular}[c]{@{}c@{}}Effective for \\out-of-distribution data leakage\end{tabular} \\ \hline
%LowKey \cite{cherepanova2021lowkey}  &NO &YES           & YES      & NO          & NO              &Not discussed\\ \hline
EM  \cite{huang2021unlearnable}    & NO&Not discussed  & NO       & NO & YES             & YES           \\ \hline
REM  \cite{fu2021robust}   &NO& Not discussed  & NO       & NO & YES             & YES           \\ \hline
OPOM \cite{zhong2022opom}   & NO& YES           & YES      & NO           & YES             & Not discussed \\ \hline
DFPP \cite{shamshad2024makeup} &NO & Not discussed&YES&NO&YES& Not discussed\\ \hline

APF  \cite{zhang2020adversarial}   &YES & Not discussed  & YES      & NO           & NO              & YES           \\ \hline
Fawkes \cite{shan2020fawkes} &YES & YES           & NO       & YES           & NO              & YES           \\ \hline
TIP-IM \cite{yang2021towards} & YES &YES           & YES      & YES           & NO              & Not discussed \\ \hline
\end{tabular}
\vspace{-0.4cm}
\end{table*}


We then compare the protection performance of the following three auxiliary data requirement methods, i.e., APF \cite{zhang2020adversarial}, Fawkes \cite{shan2020fawkes}, and TIP-IM \cite{yang2021towards}. We also adopt protection success rate (PSR) and similarity (SSIM) as the evaluation metrics. 
SSIM is a Quality-of-Experience (QoE) metric that measures variations in brightness, contrast, and structure between the original and altered images.
%对于2.2类三篇论文这一类的方法，我们进行了实验，以评估他们的性能。根据\cite{zhang2020adversarial}，\cite{shan2020fawkes}和\cite{yang2021towards}，我们使用Protection success rate和Structural similarity index作为评估指标。Protection success rate (PSR)用于评估人脸去识别是否成功。而Structural similarity index(SSIM)则是一种广泛用于测量两个图像之间差异的方法，亮度，对比度和结构三个方面进行比较。较大的SSIM意味着两个图像在结构上更相似。
%我们的实验主要使用的测试集是LFW数据集，其中包含5749个不同主题的13233张图像。为了便于进行比较，我们将图片大小统一设置为112×112×3，学习率设置为0.01，batch size为1，epoch为100。接着，基于LFW测试集，我们使用三种方法分别生成500张受保护的图像，这其中包括了500个不同的身份。最后，我们将生成的受保护图像提供给人脸识别模型ArcFace，用以测定PSR。对500张图像的原图和生成的受保护的图像进行SSIM的计算，求得平均值。实验结果展示在图中。
%根据实验结果进行比较，三种方法都有较好的性能。APF的攻击成功率较高，并且保持了很高的相似度，性能综合表现较好，TIP方法攻击成功率也较高，并且生成的图片更加自然。在图片的相似度上Fawkes的表现是最好的，但Fawkes生成了伪影，影响了视觉效果。
{\color{black}According to the original papers, we utilized the LFW dataset, which includes 13,233 images collected from 5,749 individuals in natural scenes.} To ensure consistency, we standardized the image size to 112$\times$112$\times$3, set the learning rate to 0.01, the batch size to 1, and the epoch to 100. We then generated 500 protected images, each with a unique identity, through the use of three methods. Finally, we calculated the PSA by feeding the generated protected images to the ArcFace face recognition model. The Structural Similarity Index Measure (SSIM) was applied to 500 original and generated protected images, and the average value was derived. The comparison results are presented in Fig.~\ref{fig:2} and Fig.~\ref{fig:c} (right side).
%{\color{black}The Fawkes method produces the most natural pictures with the least artifacts, which may be related to its introduction of DSSIM to measure the perceived similarity. But his protection success rate is low. APF is the opposite of Fakwes. APF has the highest protection success rate, but generates obvious distortion patterns. Due to the introduction of using MMD (maximum average difference) loss, TIP-IM shows a good balance between protection and image quality. }
It is shown that Fawkes can generate natural and artifact-free protected images, which can be attributed to its use of DSSIM for perceived similarity measurement. However, its protection success rate is low. APF has a high protection success rate but results in noticeable distortion patterns. TIP-IM strikes a balance between protection and image quality by incorporating the MMD (maximum average difference) loss.
%Fawkes方法生成的图片最自然，伪影最少，这可能与它引入了DSSIM来度量感知相似度有关。但他的保护成功率较低。APF则与Fakwes完全相反。APF的保护成功率最高，但生成了明显的失真图案。由于引入了使用MMD（最大平均差异）损失，TIP-IM在保护和图像质量之间表现出较好的权衡。



==> modelsteal/conclusion.tex <==
\section{Conclusion}
%Model extraction attacks on cloud-based MLaaS services pose serious security issues. In this article, we provide a comprehensive summary of existing methods of model extraction attacks and possible defenses. We review the latest research findings, compare advantages and disadvantages of different approaches, and conduct experimental evaluations of representative attack and defense methods. Finally, we highlight potential directions that are worth exploring to further propel the research in this field.
%The leakage of facial information on social media poses significant security risks. In this article, we provide a thorough overview of current facial privacy protection methodologies. We classify these methods into two categories and discuss each in depth. Additionally, we perform both qualitative and quantitative comparisons of various protection techniques. Furthermore, we identify unresolved issues and outline potential future research directions to further improve this field.

The leakage of facial information in cloud-based services poses significant security risks. In this article, we present a comprehensive overview of current methodologies for protecting facial image privacy. We categorize these methods into two primary approaches and provide an in-depth discussion of each. Additionally, we conduct both qualitative and quantitative evaluations of various protection techniques. Finally, we identify open challenges and propose potential future research directions to enhance privacy preservation in cloud environments.



==> modelsteal/copy.tex <==
 
\section{State-of-the-art Face Image Protection Approaches}
%{\color{black}To protect private facial information from unauthorized use by commercial deep learning models, various approaches have been proposed in recent years. Existing solutions can be divided into two categories: image obfuscation-based protection methods and adversarial perturbation-based protection methods. This classification is based on how protected images are generated. Image obfuscation techniques entail altering facial features to de-identify the face. This can involve changes in facial characteristics (e.g., gender and makeup) or blending with another image to obtain a new image. With image obfuscation-based protection methods, the resulting image may exhibit visible changes compared to the original faces. Adversarial perturbation-based protection methods add perturbations to the images to make them unlearnable to the attack model, and the perturbations are almost unrecognizable to the human eye. The protected images closely resemble the original private images.}

As the use of cloud-based services for storing and processing facial data continues to expand, the need for robust privacy protection techniques becomes more critical. To address privacy concerns in cloud environments, researchers have developed several state-of-the-art methods to protect facial images from unauthorized exploitation. These techniques are primarily categorized into image obfuscation-based protection methods and adversarial perturbation-based protection methods. Both approaches aim to preserve the utility of facial images while making them unrecognizable or ``unlearnable" to commercial face recognition models used in cloud services.



\subsection{Image Obfuscation-based Protection Methods}

%{\color{black}Based on the location of obfuscation, image obfuscation can be further divided into two categories: specific property obfuscation and whole image obfuscation.}
Image obfuscation methods alter or mask specific characteristics of facial images to make them unrecognizable to facial recognition systems. These methods typically involve modifying identifiable facial features or blending them with other visual elements to prevent accurate face identification.

\subsubsection{Specific properties obfuscation}

{\color{black} %Hu et al. \cite{hu2022protecting} introduced AMT-GAN (adversarial makeup transfer-GAN) using generative adversarial networks (GANs) to create deceptive facial images by transferring makeup from reference images, making it challenging to identify the individual's identity. Due to the application of makeup, the face appears very natural and comfortable. However, this method is primarily designed to protect female images and may not perform well on male images.

Techniques in this category focus on obfuscating certain facial attributes, such as gender, age, or skin texture. For example, AMT-GAN (Adversarial Makeup Transfer-GAN) \cite{hu2022protecting} uses generative adversarial networks (GANs) to apply makeup to a user’s face, making it difficult for face recognition models to accurately identify the individual. This method preserves the overall appearance of the face while making critical identity features difficult to detect. However, this technique is primarily effective for female faces, and adapting it for broader use cases remains a challenge. To address this challenge, Tang et al. \cite{tang2022gender} proposed Gender-AN, a gender-adversarial network that directly confuses gender to protect facial privacy. The face generator in Gender-AN undergoes optimization through a multi-task-based loss function, incorporating attribute manipulation loss, face matcher loss, adversarial loss, and reconstruction loss functions. This optimization approach ensures robust generalization performance while maintaining the natural appearance.
}



%{\color{black}To achieve more fine-grained control over the protected face while preserving the maximum utility, Chen et al. \cite{chen2022mass} introduced MaSS (multi-attribute selective suppression). MaSS enables a meticulous surgical operation on targeted data, allowing the suppression of any selected attribute while leaving the rest unchanged. It employs adversarial games between two sets of networks: one suppresses selected attributes, and the other ensures the retention of the remaining attributes.}

\subsubsection{Whole image obfuscation}


Li et al. \cite{li2021deepblur} proposed DeepBlur, which blurs images in the latent space of a pre-trained generative model capable of creating realistic facial images. The process involves three steps: latent representation search, deep blurring, and image generation. The input face image is transformed into a latent space vector, modified multiple times using a pre-trained model to remove identifying information, and then a realistic face is generated based on the blurred latent space vector model. This approach allows for generating different levels of obfuscation for various applications. However, there is a noticeable visual gap between the generated and original images.

%He et al. \cite{he2024diff} proposed Diff-Privacy, which is a diffusion-based method for facial privacy protection by using advanced diffusion models to anonymize images in cloud-based environments. This approach ensures that facial images are unlearnable by recognition models while maintaining visual quality. The flexibility of this method allows it to meet diverse privacy protection requirements in cloud services.

%In addition to these software-based solutions, Lopez et al. \cite{lopez2024privacy} presented a hardware-level approach to facial privacy protection, using optical encoders to generate face heatmaps that hide identities while preserving the rest of the image for use in cloud-based environments. Such advancements provide another layer of protection, offering a more robust defense against identity-based recognition systems.}

%He et al. \cite{he2024diff} introduced Diff-Privacy, a diffusion-based method for facial privacy protection that leverages advanced diffusion models to anonymize images, particularly in cloud-based environments. Diff-Privacy ensures that facial images become ``unlearnable" by recognition models, while still maintaining a high degree of visual fidelity. This method is particularly flexible, making it well-suited for a wide range of privacy protection needs in cloud services. Its ability to maintain both privacy and visual quality positions it as a robust solution for modern privacy challenges.




{\color{red}He et al. \cite{he2024diff} introduced Diff-Privacy, a more advanced diffusion-based method for anonymizing facial images in cloud-based environments. Diffusion models, originally designed for image generation and restoration, incrementally add noise to an image and then reverse the process to recover or generate a new image. In Diff-Privacy, this diffusion process is employed to introduce noise into facial images in such a way that the images remain unrecognizable by facial recognition systems. Unlike DeepBlur, which directly manipulates the latent space, Diff-Privacy operates at the pixel level to iteratively transform the image. The method maintains high visual fidelity while making the facial data ``unlearnable" by machine learning models. This flexibility allows it to meet varying privacy requirements in cloud-based services, where balancing visual quality and data privacy is critical.

In addition to software-based solutions, Lopez et al. \cite{lopez2024privacy} presented a hardware-level approach to facial privacy protection through the use of optical encoders. Their method generates face heatmaps that obscure the user's identity while preserving other aspects of the image for non-sensitive applications. This hardware-level solution adds another layer of protection, offering a more robust defense against identity-based recognition systems by directly addressing the vulnerabilities that software-based solutions may overlook in cloud environments.

Zhang et al. \cite{zhangtransferable} further addressed the issue of Blind Face Restoration (BFR), where obfuscated facial images could be restored using advanced restoration models. Their transferable adversarial obfuscation method creates obfuscated images that resist restoration attempts by BFR models. This method enhances the generalization of obfuscated faces across various BFR models, ensuring that even if adversaries attempt to retrain restoration models on obfuscated images, the obfuscation remains effective. This technique is particularly valuable in scenarios where attackers have access to BFR systems and aim to reverse facial obfuscation.


}


%Different from AnonymousNet, UP-GAN (utility-preserving GAN) \cite{Hao2019UPGAN} operates solely on the utility information and does not require direct access to the original facial data. Utility information is defined based on facial properties like age, gender, skin tone, pose, and expression. To obscure faces, UP-GAN initially uses an auxiliary system to detect utility information. The fake face is then generated by the UP-GAN model using such information. Since the generated face has the same pose and expression, it can be swapped with the original face using face-swapping algorithms to perform de-identification. UP-GAN preserves a variety of soft biometrics that do not display identity and also achieves k-anonymity.


%To enhance the similarity between the generated and original images, Wu et al. \cite{wu2019PPGAN} introduced PP-GAN (privacy-protective GAN). PP-GAN includes a verificator to eliminate biometric information and a regulator to preserve image utility within the GAN network. It removes biometric details while preserving image quality, including brightness, contrast, and structural similarity. The regulator ensures the consistency between the generated image and the original image by utilizing the pixel-level structure similarity measured through SSIM. However, PP-GAN does not consider k-anonymity privacy protection, leaving the privacy of the entire dataset vulnerable. k-anonymity is a privacy technique in data anonymization. It ensures that individuals in a dataset are not easily distinguishable from at least k-1 other individuals based on certain attributes, aiming to protect individual privacy by making it difficult for adversaries to identify specific people in the dataset.

%Li et al. \cite{AnonymousNet} proposed AnonymousNet as an alternative method that obfuscates facial identities while generating realistic images. This method achieves k-anonymity privacy protection, and it consists of four key steps: facial feature extraction, semantic-based attribute obfuscation, de-identified face generation, and adversarial perturbation. The process begins by utilizing a large number of attribute classifiers to recognize facial attributes. After attribute obfuscation, AnonymousNet utilizes GAN to generate a new facial image with modified attributes. Finally, AnonymousNet adds a kind of antagonistic noise to the generated image to achieve better performance.AnonymousNet can generate realistic images with fake identities and balance privacy and usability in quality and quantity. However, AnonymousNet requires access to the original face data, which may lead to privacy disclosure.


\subsection{Adversarial Perturbation-based Protection Methods}

Adversarial perturbation techniques focus on adding subtle, imperceptible noise to facial images, making them resistant to recognition by machine learning models without significantly altering the visual quality of the image. These perturbations ensure that even if the images are used to train a face recognition model, the model will fail to learn meaningful representations from the data.

{\color{black}We divide the schemes of adversarial perturbation into two categories according to whether requiring auxiliary data or not.}
%Unlike image obfuscation-based methods, which may visibly alter the original images, Adversarial perturbation-based protection methods add perturbations to the images to make them unlearnable to the attack model, and the perturbations are almost unrecognizable to the human eye. The generated protected images are almost the same as the original private image.


\subsubsection{Non-auxiliary data requirement} 

{\color{black} Under such a protection paradigm, the defenders do not rely on any auxiliary dataset to protect the private faces.}
%{\color{black}Cherepanova et al. \cite{cherepanova2021lowkey} proposed LowKey, which protects users from unauthorized surveillance and is made available to the public as a network tool. LowKey alters private faces to create a perturbed version that does not match probe images of the same person. It achieves this by moving the feature space far from the protected image while minimizing perceptual similarity loss. LowKey is the first evasion tool against Amazon Rekognition and the Microsoft Azure Face Recognition APIs. However, it will exhibit visual artifacts and distortions perceptible to the human eye, impacting image quality.
%In addition to generating perturbation for a single image, defenders can generate universal perturbation that can be applied to a specific category, known as class-wise noise. 
Huang et al. \cite{huang2021unlearnable} generated unlearnable examples that contain error-minimizing noises, referred to as EM. It is based on such an intuition: the samples with larger training loss may contain more knowledge to be learned. Generating optimal perturbations that minimize the loss can suppress the informative knowledge of the data, thereby protecting the data from being learned. %Although class-wise noise is much more convenient and efficient, it is more likely to be evaded by adversarial training. To address this challenge,
Further, Fu et al. \cite{fu2021robust} introduced REM (robust error-minimizing noise), which effectively reduces the adversarial training loss and suppresses the learnable knowledge of data in adversarial training.

{\color{black}Zhong et al. \cite{zhong2022opom} presented OPOM (one person one mask) to generate class-wise masks by optimizing each training sample in a direction away from the feature subspace of the protected face image. {\color{black}The feature subspace represents the specific set of features or representations associated with that face, often determined by techniques like class centers, convex hulls, and affine hulls.} OPOM is efficient and suitable for real-time privacy protection applications. However, OPOM may not be effective in scenarios where there are significant differences between the testing images and the training samples, such as larger poses, different illumination, or different occlusions compared to the original protected image.} 

{\color{red}Shamshad et al. \cite{shamshad2024makeup} introduced DFPP, which leverages makeup as an adversarial technique to obfuscate identity in facial images. DFPP employs a deep neural network to transfer makeup features from a reference image to a target image, effectively masking the user's identity while preserving the visual aesthetics. This method is particularly effective in black-box facial recognition environments, where the internal workings of the recognition model are unknown. Although makeup is the medium, the technique generates adversarial perturbations that disrupt the recognition model, making it fall under adversarial perturbation-based methods rather than specific property obfuscation.}

\cite{zhangtransferable}

\begin{figure}[tt]
\vspace{-0.4cm}
	\centering
	\includegraphics[width=9cm]{modelsteal/Figure_1 (1).png}\\
	\caption{Comparison of facial privacy protection performance of EM \cite{huang2021unlearnable}, REM \cite{fu2021robust}, and OPOM \cite{zhong2022opom}.}
    \label{fig:fl}
    \vspace{-0.4cm}
\end{figure}

\begin{figure}[tt]
	\centering
	\includegraphics[width=9cm]{modelsteal/fig.png}\\
	\caption{Comparison of facial privacy protection performance of APF \cite{zhang2020adversarial}, Fawkes \cite{shan2020fawkes}, and TIP-IM \cite{yang2021towards}.}
    \label{fig:2}
    \vspace{-0.6cm}
\end{figure}

\begin{figure*}[tt]
	\centering
	\includegraphics[width=15cm]{c.png}\\
	\caption{Visual comparison results of different facial privacy protection methods.}
    \label{fig:c}
    \vspace{-0.6cm}
\end{figure*}

\iffalse
\begin{figure*}[tt]
	\centering
	%\hspace{-0.8cm}
	\begin{minipage}[t]{3.24in}
		\centering
		\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=3.24in]{b.png}\\
		\centerline{\footnotesize (a) }
	\end{minipage}
	\hspace{-0cm}
	\begin{minipage}[t]{2.61in}
		\centering
		\includegraphics[trim=0mm 0mm 0mm 0mm, clip,width=2.61in]{a.png}\\
		\centerline{\footnotesize (b)}
	\end{minipage}
	\hspace{-0cm}
	
	\caption{{\color{black} Visual comparison results of different facial privacy protection methods.}} \label{fig:c}
\end{figure*}
\fi



\subsubsection{Auxiliary data requirement}

{\color{black}In this case, the defender protects private faces with the assistance of an auxiliary dataset.}

%requires an auxiliary dataset to generate the adversarial perturbation.}
%generate the image-independent universal adversarial perturbation or select a target category from it to generate a perturbed image.

{\color{black}
Zhang et al. \cite{zhang2020adversarial} developed APF (adversarial privacy-preserving filter) to protect online shared face images from unauthorized use. APF is an end-cloud collaborated adversarial attack framework and ensures that only users' own devices can access the original images. It involves three key modules: image-specific gradient generation, adversarial gradient transfer, and universal adversarial perturbation enhancement. Image-specific gradient generation extracts gradients on the user end, and adversarial gradient transfer fine-tunes them in the server cloud. The server creates a universal perturbation by maximizing feature distances in an auxiliary dataset. An enhancement module adjusts it to match the image-specific perturbation for better integration.}
{\color{black}In the same period, Shan et al. \cite{shan2020fawkes} proposed Fawkes. In Fawkes, the defender first selects a target category from a publicly auxiliary dataset. Specifically, the authors use a feature extractor to calculate the centroid of the feature space for each candidate class and pick the class whose feature representation centroid is the most dissimilar to the feature representation of all the private images. Then Fawkes randomly selects an image from the target class and optimizes the calculation of the small disturbance of the protected image. In this step, the authors introduced DSSIM (Structural Dissimilarity Index) to ensure that the processed image is visually similar to the original image. However, Fawkes is designed for the white box, requiring access to the feature extractor the user wishes to subvert.}

{\color{black}Unlike Fawkes, Yang et al. \cite{yang2021towards} introduced TIP-IM (targeted identity-protection iterative method) to encrypt private facial images, offering privacy protection against black-box face recognition systems. TIP-IM generates adversarial identity masks and overlays them on facial images, concealing the original identities without compromising visual quality. To create the adversarial identity masks, the authors employ a novel optimization mechanism, using MMD (Max Mean Discrepancy) loss to enhance the visual quality of the crafted adversarial examples. This allows concealing the original images without sacrificing their visual quality, and the generated masks are effective for other black-box models. To control the misclassification results, the authors use greedy insertion to select the optimal victim image from an auxiliary dataset. However, as TIP-IM lacks constraints on visual behavior, except for naturalness defined by MMD, the increase in noise intensity may not guarantee a natural change in pixel information, especially when the de-identification effect dominates naturalness in the face image.}




==> modelsteal/evaluations.tex <==
 
\section{State-of-the-art Face Image Protection Approaches}

As the use of cloud-based services for storing and processing facial data continues to expand, the need for robust privacy protection techniques becomes more critical. To address privacy concerns in cloud environments, researchers have developed several state-of-the-art methods to protect facial images from unauthorized exploitation. These techniques are primarily categorized into image obfuscation-based protection methods and adversarial perturbation-based protection methods. Both approaches aim to preserve the utility of facial images while making them unrecognizable or ``unlearnable" to commercial face recognition models used in cloud services.



\subsection{Image Obfuscation-based Protection Methods}
Image obfuscation methods alter or mask specific characteristics of facial images to make them unrecognizable to facial recognition systems. These methods typically involve modifying identifiable facial features or blending them with other visual elements to prevent accurate face identification.

\subsubsection{Specific properties obfuscation}
Techniques in this category focus on obfuscating certain facial attributes, such as gender, age, or skin texture. For example, AMT-GAN \cite{hu2022protecting} uses generative adversarial networks (GANs) to apply makeup to a user’s face, making it difficult for face recognition models to accurately identify the individual. This method preserves the overall appearance of the face while making critical identity features difficult to detect. However, this technique is primarily effective for female faces, and adapting it for broader use cases remains a challenge. To address this challenge, Tang et al. \cite{tang2022gender} proposed Gender-AN, a gender-adversarial network that directly confuses gender to protect facial privacy. The face generator in Gender-AN undergoes optimization through a multi-task-based loss function, incorporating attribute manipulation loss, face matcher loss, adversarial loss, and reconstruction loss functions. This optimization approach ensures robust generalization performance while maintaining the natural appearance.

\subsubsection{Whole image obfuscation}
Li et al. \cite{li2021deepblur} proposed DeepBlur, which blurs images in the latent space of a pre-trained generative model capable of creating realistic facial images. The process involves three steps: latent representation search, deep blurring, and image generation. The input face image is transformed into a latent space vector, modified multiple times using a pre-trained model to remove identifying information, and then a realistic face is generated based on the blurred latent space vector model. This approach allows for generating different levels of obfuscation for various applications. However, there is a noticeable visual gap between the generated and original images.

He et al. \cite{he2024diff} introduced Diff-Privacy, a more advanced diffusion-based method for anonymizing facial images in cloud-based environments. Diffusion models, originally designed for image generation and restoration, incrementally add noise to an image and then reverse the process to recover or generate a new image. In Diff-Privacy, this diffusion process is employed to introduce noise into facial images in such a way that the images remain unrecognizable by facial recognition systems. Unlike DeepBlur, which directly manipulates the latent space, Diff-Privacy operates at the pixel level to iteratively transform the image. The method maintains high visual fidelity while making the facial data ``unlearnable" by machine learning models. This flexibility allows it to meet varying privacy requirements in cloud-based services, where balancing visual quality and data privacy is critical.

In addition to software-based solutions, Lopez et al. \cite{lopez2024privacy} presented a hardware-level approach to facial privacy protection through the use of optical encoders. Their method generates face heatmaps that obscure the user's identity while preserving other aspects of the image for non-sensitive applications. This hardware-level solution adds another layer of protection, offering a more robust defense against identity-based recognition systems by directly addressing the vulnerabilities that software-based solutions may overlook in cloud environments.

Zhang et al. \cite{zhangtransferable} further addressed the issue of Blind Face Restoration (BFR), where obfuscated facial images could be restored using advanced restoration models. Their transferable adversarial obfuscation method creates obfuscated images that resist restoration attempts by BFR models. This method enhances the generalization of obfuscated faces across various BFR models, ensuring that even if adversaries attempt to retrain restoration models on obfuscated images, the obfuscation remains effective. This technique is particularly valuable in scenarios where attackers have access to BFR systems and aim to reverse facial obfuscation.





\subsection{Adversarial Perturbation-based Protection Methods}

Adversarial perturbation techniques focus on adding subtle, imperceptible noise to facial images, making them resistant to recognition by machine learning models without significantly altering the visual quality of the image. These perturbations ensure that even if the images are used to train a face recognition model, the model will fail to learn meaningful representations from the data. We divide the schemes of adversarial perturbation into two categories according to whether requiring auxiliary data or not.

\subsubsection{Non-auxiliary data requirement} 

{\color{black} Under such a protection paradigm, the defenders do not rely on any auxiliary dataset to protect the private faces.}
Huang et al. \cite{huang2021unlearnable} generated unlearnable examples that contain error-minimizing noises, referred to as EM. It is based on such an intuition: the samples with larger training loss may contain more knowledge to be learned. Generating optimal perturbations that minimize the loss can suppress the informative knowledge of the data, thereby protecting the data from being learned. 
Further, Fu et al. \cite{fu2021robust} introduced REM (robust error-minimizing noise), which effectively reduces the adversarial training loss and suppresses the learnable knowledge of data in adversarial training.

{\color{black}Zhong et al. \cite{zhong2022opom} presented OPOM (one person one mask) to generate class-wise masks by optimizing each training sample in a direction away from the feature subspace of the protected face image. {\color{black}The feature subspace represents the specific set of features or representations associated with that face, often determined by techniques like class centers, convex hulls, and affine hulls.} OPOM is efficient and suitable for real-time privacy protection applications. However, OPOM may not be effective in scenarios where there are significant differences between the testing images and the training samples, such as larger poses, different illumination, or different occlusions compared to the original protected image.} 

Shamshad et al. \cite{shamshad2024makeup} introduced DFPP, which leverages makeup as an adversarial technique to obfuscate identity in facial images. DFPP employs a deep neural network to transfer makeup features from a reference image to a target image, effectively masking the user's identity while preserving visual aesthetics. This method is particularly effective in black-box facial recognition environments, where the internal workings of the recognition model are unknown. Although makeup is the medium, the technique generates adversarial perturbations that disrupt the recognition model, making it fall under adversarial perturbation-based methods rather than specific property obfuscation.

%\cite{zhangtransferable}

\begin{figure}[tt]
\vspace{-0.4cm}
	\centering
	\includegraphics[width=9cm]{modelsteal/PSR_SSIM_Comparison.pdf}\\
	\caption{Comparison of facial privacy protection performance of EM \cite{huang2021unlearnable}, REM \cite{fu2021robust}, and OPOM \cite{zhong2022opom}.}
    \label{fig:fl}
    \vspace{-0.4cm}
\end{figure}

\begin{figure}[tt]
	\centering
	\includegraphics[width=9cm]{modelsteal/PSR_SSIM_Comparison2.pdf}\\
	\caption{Comparison of facial privacy protection performance of APF \cite{zhang2020adversarial}, Fawkes \cite{shan2020fawkes}, and TIP-IM \cite{yang2021towards}.}
    \label{fig:2}
    \vspace{-0.6cm}
\end{figure}

\begin{figure*}[tt]
	\centering
	\includegraphics[width=13cm]{c.png}\\
	\caption{Visual comparison results of different facial privacy protection methods.}
    \label{fig:c}
    \vspace{-0.6cm}
\end{figure*}



\subsubsection{Auxiliary data requirement}

{\color{black}In this case, the defender protects private faces with the assistance of an auxiliary dataset.}

%requires an auxiliary dataset to generate the adversarial perturbation.}
%generate the image-independent universal adversarial perturbation or select a target category from it to generate a perturbed image.

{\color{black}
Zhang et al. \cite{zhang2020adversarial} developed APF (adversarial privacy-preserving filter) to protect online shared face images from unauthorized use. APF is an end-cloud collaborated adversarial attack framework and ensures that only users' own devices can access the original images. It involves three key modules: image-specific gradient generation, adversarial gradient transfer, and universal adversarial perturbation enhancement. Image-specific gradient generation extracts gradients on the user end, and adversarial gradient transfer fine-tunes them in the server cloud. The server creates a universal perturbation by maximizing feature distances in an auxiliary dataset. An enhancement module adjusts it to match the image-specific perturbation for better integration.}
{\color{black}In the same period, Shan et al. \cite{shan2020fawkes} proposed Fawkes. In Fawkes, the defender first selects a target category from a publicly auxiliary dataset. Specifically, the authors use a feature extractor to calculate the centroid of the feature space for each candidate class and pick the class whose feature representation centroid is the most dissimilar to the feature representation of all the private images. Then Fawkes randomly selects an image from the target class and optimizes the calculation of the small disturbance of the protected image. In this step, the authors introduced DSSIM (Structural Dissimilarity Index) to ensure that the processed image is visually similar to the original image. However, Fawkes is designed for the white box, requiring access to the feature extractor the user wishes to subvert.}

{\color{black}Unlike Fawkes, Yang et al. \cite{yang2021towards} introduced TIP-IM (targeted identity-protection iterative method) to encrypt private facial images, offering privacy protection against black-box face recognition systems. TIP-IM generates adversarial identity masks and overlays them on facial images, concealing the original identities without compromising visual quality. To create the adversarial identity masks, the authors employ a novel optimization mechanism, using MMD (Max Mean Discrepancy) loss to enhance the visual quality of the crafted adversarial examples. This allows concealing the original images without sacrificing their visual quality, and the generated masks are effective for other black-box models. To control the misclassification results, the authors use greedy insertion to select the optimal victim image from an auxiliary dataset. However, as TIP-IM lacks constraints on visual behavior, except for naturalness defined by MMD, the increase in noise intensity may not guarantee a natural change in pixel information, especially when the de-identification effect dominates naturalness in the face image.}




==> modelsteal/future.tex <==
\section{Future Research Directions}

\subsection{Potential Research Directions on Image Obfuscation-based Protection Methods}

We propose the following research directions for enhancing the performance of image obfuscation-based protection methods.

First, it is shown that the facial images generated through image obfuscation sometimes can have a noticeable departure from the original image. Excessive modifications to facial features can have a negative effect on user experience. To improve the application, a more targeted approach that only changes the identity-relevant aspects of the face is needed. Further research should identify key facial characteristics impacting identity and modify those areas for greater privacy protection.

%Second, current make-up-based image perturbation techniques \cite{hu2022protecting} primarily concentrate on safeguarding the facial images of women. There is a need for further exploration to design a make-up-based facial protection method that is effective for men.

Second, makeup-based image perturbation methods \cite{hu2022protecting} have been primarily designed for female facial images. However, effective privacy protection should be universal. There is a need to expand these techniques to be equally effective for male facial images. Future research could explore gender-neutral perturbation techniques or develop makeup-based protection methods that work across different genders.



Third, image obfuscation will inevitably alter the appearance of facial images, thus causing visible artifacts. To effectively preserve privacy, face de-recognition methods should generate facial images that maintain a natural look and retain key facial features. Further research is needed to reduce the artifacts produced by these techniques.


Finally, existing facial privacy protection methods mainly focus on static photos. However, there is a research gap in protecting privacy in videos, which are dynamic and composed of multiple frames. How to design effective privacy protection methods for videos requires further exploration. 



\subsection{Potential Research Directions on Adversarial Perturbation-based Protection Methods}

We propose the following avenues for exploration in the area of face privacy protection using adversarial perturbations.

Firstly, most current methods focus on selfies, which are clear and upright portraits. However, surveillance cameras capture people in varying light and occlusion conditions in reality. To better reflect real-life scenarios, future research should consider more challenging environments for face recognition. %Additionally, %as the extracted features may be limited, 
Additionally, it's crucial to consider privacy protection beyond static images, extending to dynamic video fields. Researchers may consider using advanced algorithms for face alignment or employing super-resolution methods to enhance key features such as the eyes.

Second, adversarial perturbation-based privacy protection methods often lead to image quality degradation. It is important to ensure that the protected image maintains a good visual experience. Future research should design protection tools that do not negatively impact the visual experience of users. For instance, instead of relying on traditional norms such as the $L_2$ and $L_\infty$ norm, researchers may consider alternative constraints such as reducing the number of modified pixels or even trying the one-pixel attack approach.

Third, to make the protection methods accessible to users, the time cost of generating protected images must be reasonable.
A potential research direction is to improve the noise generation process for higher efficiency. A potential solution is to restrict noise distribution to specific areas, such as the face's position and size, rather than adding noise to the entire image.

{\color{black}Lastly, in the future, new attack threats may emerge that can circumvent current privacy protection measures. While existing defensive perturbations have proven effective, in real-world training at commercial companies like Google and Alibaba, expert trainers often include pre-processing procedures (e.g., data augmentation) in collected samples to improve model performance. Data augmentation enhances both data quantity and adversarial robustness. To this end, these protected faces might still be identifiable to face recognition models after advanced augmentation. Moreover, adversarial training during the training process may also weaken existing protection. It is essential to address these potential challenges and develop more comprehensive and long-term protection plans.}






==> modelsteal/intro.tex <==
\section{Introduction}
%The rapid development of face recognition technology has greatly facilitated people's daily lives. In recent years, face recognition has been fully utilized in many fields, such as payment, mobile phone unlocking, and access control. {\color{black}However, social media users willingly share their facial images on online social networks (OSNs) \cite{fei2024online}, such as Facebook, Twitter, MySpace, Flickr, and Youtube, making them accessible for scraping. Such ``free" data can be highly valuable for commercial organizations to train face recognition (FR) models and use for authentication. Large-scale photo analysis not only reveals user identities but also allows inference of user relationships. Besides, it also raises the risk of deepfake attacks, producing realistic fake videos or images with facial data that can lead to identity theft, misinformation, and other harmful activities. To safeguard the facial privacy of social media users, there is a need for a secure method to release their data on online social networks, preventing unauthorized use of uploaded face images.}

%The rapid advancement of facial recognition technology has significantly enhanced convenience in various applications, including payment systems, mobile device unlocking, and access control \cite{shivanna2024biometric}. Cloud-based services, which handle and store vast amounts of user data, have increasingly integrated facial recognition systems to streamline these processes. However, as more users rely on cloud platforms for data storage and processing, their facial images become vulnerable to unauthorized access, misuse, and exploitation. In particular, cloud service providers often store facial images for purposes such as identity verification, model training, and user authentication, raising significant concerns regarding data privacy and security \cite{zhang2024validating}.



%The large-scale collection and analysis of facial images in cloud environments not only facilitate identity recognition but also introduce significant risks. Unauthorized access to this sensitive data can lead to privacy violations such as the creation of deepfakes, identity theft, and other malicious activities. These risks are further exacerbated in cloud platforms, where data is often shared across multiple entities and geographical regions, complicating users' ability to control how their facial data is utilized.

The rapid growth of facial recognition technology has greatly improved convenience in applications like payment systems, mobile device unlocking, and access control \cite{shivanna2024biometric}. Cloud-based services, which store and process large amounts of user data, increasingly integrate facial recognition to streamline these functions. However, as users depend more on cloud platforms, their facial images face heightened risks of unauthorized access, misuse, and exploitation. Cloud service providers often retain facial images for purposes such as identity verification, model training, and user authentication, raising serious concerns about data privacy and security \cite{zhang2024validating}.

The extensive collection of facial images in cloud environments facilitates identity recognition but also introduces significant privacy risks. Unauthorized access to this sensitive data can result in deepfake creation, identity theft, and other malicious activities. These risks are further amplified in cloud platforms, where data is frequently shared across multiple entities and regions, making it harder for users to control how their facial data is used.



%Research has demonstrated that these models can be used to identify social media users and track user relationships through large-scale photo analysis. And some private information of the users, including names and emails, can be inferred from the well-trained model. To safeguard the facial privacy of social media users, there needs to be a way to safely release their data on online social networks, preventing unauthorized use of uploaded face images.
%without allowing third parties to train FR models using these data.
\begin{figure}[tt]
	\centering
	\includegraphics[width=8.4cm]{modelsteal/overview.png}\\
	\caption{{\color{black}Protecting private facial privacy from unauthorized exploitation in cloud-based services. }}
    \label{fig:overview}
    \vspace{-0.6cm}
\end{figure}

%{\color{black}There is a long line of works \cite{zhong2022opom,hu2022protecting, chen2022mass, tang2022gender, cherepanova2021lowkey, yang2021towards,AnonymousNet,li2021deepblur} exploring how to protect social media users’ facial privacy from exploitation. A schematic diagram of social media users' facial privacy protection process is shown in Fig. \ref{fig:overview}. Before publishing private facial photos on social media platforms, users may choose to add perturbations to these photos to make them ``unlearnable'' by commercial face recognition models. Even if crawling amounts of these protected samples, the face recognition model's performance remains comparable to random guessing when attempting to recognize a new photo (probe image) of the same individual. Preserving users' facial privacy without compromising their photo-sharing experience requires addressing both privacy and utility. Privacy involves ensuring the user's identification information is unrecognizable in the shared face images, while utility focuses on maintaining the visual quality of the face images. To achieve this, users can add imperceptible noises to private photos, employ makeup techniques, and blend them with other public photos containing different biological information.}


There is a significant body of research exploring how to protect the privacy of facial images stored and processed in cloud-based services \cite{zhong2022opom, hu2022protecting, yang2021towards,li2021deepblur}. Before uploading private facial photos to cloud platforms for storage or processing, users can add perturbations to these images to make them ``unlearnable" by commercial face recognition models. Even when large volumes of such protected images are processed in the cloud, the performance of face recognition models degrades to a level similar to random guessing when attempting to recognize a new photo (probe image) of the same individual. Preserving users' facial privacy while ensuring the functionality involves addressing both privacy and utility concerns. Privacy entails making the user's identification information unrecognizable in the uploaded face images, while utility focuses on maintaining the visual and functional quality of these images. To strike this balance, users can apply imperceptible noise to their facial images, utilize makeup techniques, or blend their facial features with other publicly available images to mask identifying characteristics.

%To achieve this balance, users can add imperceptible noise to their private photos, apply makeup techniques, or blend their facial data with other publicly available images containing different biological features.


In this article, we present a comprehensive and systematic review of methods for preserving facial image privacy in cloud-based services. We categorize facial privacy protection methods into two main types: image obfuscation-based methods and adversarial perturbation-based methods, based on how the protected images are generated. We summarize the strengths and weaknesses of these techniques and provide qualitative and quantitative comparisons of various approaches. Finally, we identify key challenges and propose future research directions to further enhance privacy protection in cloud computing environments.




%In this article, we demonstrate a comprehensive and systematic review of methods for protecting social media users' facial privacy. {\color{black}We categorize facial privacy protection methods into two types: image obfuscation-based and adversarial perturbation-based. This classification is based on how protected images are generated.} We not only summarize the methods of these protection methods but also discuss their pros and cons. Through qualitative analysis and experimental evaluations, we provide in-depth comparisons of various facial privacy protection techniques. Finally, we identify open challenges and suggest potential future research directions for advancing this field.





==> modelsteal/name.tex <==
 
\section{Attacks and Defenses approaches}
In this section, we present a thorough investigation on the existing approaches of the model extraction attacks and defenses on the cloud-based models. We first classify them according to their theoretical background, then briefly describe their technical implementation details.

\subsection{Attacks Approaches}
According to the purposes of the attacker, we classify the state-of-the-art attack schemes into two categories: model attributes extraction and model functionality extraction.
\subsubsection{Model Attributes Extraction}
Nowadays, most of the extraction attack focus on attributes stealing (i.e., parameters \cite{tramer2016stealing}, hyperparameters \cite{wang2018stealing}, architecture \cite{duddu2018stealing}, and decision boundary \cite{juuti2019prada}) which are tightly related to the intellectual property rights of the cloud-based models.


Tramer et al. proposed StealML \cite{tramer2016stealing} that works on various popular cloud-based models such as logistic regression, SVM, decision tree, and shallow neural networks. It can efficiently steal the internal parameters of a black-box ML model from its prediction outputs with confidence scores. Firstly, the attacker uses a set of crafted or publicly available samples to obtain corresponding outputs $f\left (x \right )$ by querying the cloud-based model multiple times. Furthermore, he uses the input-output pairs $\left (x, f\left (x \right )\right )$ to construct a set of equations. Though solving the equations of parameters, the adversary can infer extract model parameters. Such attack is conceptually simple, but it needs to know the model family. Moreover, it only applies to simple models with small amounts of parameters and is ineffective for DNN models, which makes it a limited algorithm.


Apart from parameters, hyperparameters inside the cloud-based ML models are also of significant importance and commercial value. Wang et al. proposed StealHyperparameter \cite{wang2018stealing} to deal with the hyperparameters extraction challenges. It is based on the observation that ML algorithms determine model parameters via minimizing the objective function, and the \emph{gradient} of the objective function at the learnt model parameters is close to 0. Hence, the adversary can compute the gradient of the objective function at the model parameters and set it to 0 to obtain a system of linear equations about the hyperparameters. But, because the number of equations is generally larger than the number of unknown variables, this linear system is usually overdetermined (i.e., the number of model parameters is larger than the hyperparameters). Therefore, the authors leveraged the \emph{linear least square method} \cite{montgomery2012introduction} to estimate the hyperparameters. 


To infer the architecture of a Neural Network, Duddu et al. proposed StealNN \cite{duddu2018stealing} using the techniques of timing side channels. It is based on the truth that the total execution time of the neural network depends on the depth of the network. Besides, it assumes the adversary knows the victim's hardware and can possess the same device aiming to build timing profiles of different neural networks. Specifically, the attacker first uses iterative membership inference \cite{salem2018ml} to reconstruct its training dataset $D_{T}$, and queries the targeted model to calculate the total execution time. Then he trains a regressor on $D_{A}$ = $ \left \{ \left (T_{1},K_{1} \right ),\cdots, \left (T_{N},K_{N} \right ) \right \}$, i.e., the variation of execution time $ \left (T \right ) $ with neural network depth $\left(k\right )$. Finally, the attacker can infer the depth (the number of layers) of the DNN using the pre-trained regressor and the total execution time.




Recently, Juuti et al. \cite{juuti2019prada} presented a novel iterative model extraction strategy that includes many duplication rounds, namely PRADA. Each round consists of three phases: queries the cloud-based model $F$, trains substitute model $F'$ on the obtained labels $F(x)$, and crafts new synthetic samples based on Jacobian-Based Data Augmentation (JBDA) using the updated $F'$. Especially to deserve to be mentioned, different from other extraction methods above, one of the attack success metrics of such scheme is the transferability of the \emph{adversarial sample}, which considers extracting the decision boundary of the targeted black-box model.



\subsubsection{Model Functionality Extraction.}
Apart from the attributes extraction, another attack goal is only to construct a substitute model that can compete with the targeted cloud-based model at the same task, i.e., functionality attacks.

Shi et al. proposed StealClassifier \cite{shi2017steal} to extract the functionality of a Naive Bayes and SVM text classification classifier in the context of text classification. In this method, the authors leveraged DNN architecture to approximate the functionality of the above basic machine learning models. And they showed that the reverse is impractical, i.e., using SVM or Naive Bayes models to extract the functionality of DNN architectures.

To steal the functionality of more complex architecture, i.e., DNN models, KnockoffNets \cite{orekondy2019knockoff} is proposed. The overall phases include three parts: substitute model architecture selected, transfer dataset construct, and train the substitute model. Since the architecture of the cloud-based model is unknown to the attacker, selecting the same architecture is not a trivial thing. Fortunately, the existing theory is proved that a proper complexed architecture is enough for extracting the functionality of the common DNN model \cite{papernot2017practical,orekondy2019knockoff} even not in the same series (e.g., VGG-16 extract ResNet-10). As for the transfer dataset (i.e., image-prediction pairs) construct, the authors queried a very large benchmark datasets (e.g., ILSVRC, OpenImages) to the cloud-based model to obtain the labels. To query more efficiently, this method leverages \emph{reinforcement learning} strategies to select the best samples to query. Finally, the attacker can obtain a knockoff model after training on the transfer dataset using the selected architecture. Although it is proved effective to replicate a mature commercial API, it requires access to large sets of natural samples, which is not comparable to the synthetic samples using in \cite{juuti2019prada,papernot2017practical}.



\subsection{Defenses Approaches}

In this part, we introduce two state-of-the-art countermeasures against model extraction attacks: defending by output perturbation (i,e., injects a targeted perturbation to the model predictions) and detecting by observing the query (i.e., monitors user-server streams and generates a warning if detecting malicious behavior).
 
\subsubsection{Defence by output perturbations}

Lee \emph{et al.} proposed Deceptive Perturbations \cite{lee2019defending}, which perturbs the softmax activation function (i.e., produces the output probability) to make the attacker away from targeted parameters. Specifically, it alters original response to $\hat{y}^{i}$ in $j$-th dimension with a sum-to-one normalizer $\alpha ^{i}$: $\hat{y}^{i}_{j}= \alpha ^{i}\left ( y^{i} _{j}-r\left ( y^{i} _{j} \right )\right )$, $\hat{y}^{i}_{k}\geq \hat{y}^{i}_{j}$ for $j= 1,...,K$, where $r\left ( y^{i} _{j} \right )$ is a perturbation function called Reverse Sigmoid \cite{lee2019defending}. However, such remedy maintains the accuracy of top-1 label leading to some extraction attacks (i.e., work while discard prediction probabilities) are still effective \cite{orekondy2019knockoff,juuti2019prada}.


Based on the problem above, Orekondy \emph{et al.} proposed Prediction Poisoning \cite{orekondy2019prediction}. It is the first utility-constrained defense framework to satisfy both privacy and utility objective via introducing targeted perturbations to predictions,
that is: $\tilde{y} = \left ( 1-\alpha  \right )y+\alpha y^{*}$. 
The poisoning probability distribution $y^{*}$ satisfies the objective of mistraining the substitute model though maximizing the angular deviation between the gradient signals of poisoned posteriors and that of the original model. While $\alpha$ is a tunable parameter selected to meet accuracy-preserving utility objective $dist\left ( y,\tilde{y} \right )\leq \epsilon $, where $\epsilon$ is perturbation magnitude. The defender can trade off the utility and the security by varying $\alpha$. However, such a method requires multiple gradient computations, which results in calculation costs and inference delays increasing by orders of magnitude.


Another countermeasure is to use differential privacy to perturb the output, named BDPL \cite{zheng2019bdpl}. It appends a boundary differential private layer to perturb query response working around the decision boundary. Specifically, first it identifies whether a query $x_{q}$ is sensitive by checking corner points with projected interval $\Delta _{i}$ to $x_{q}$ on all dimension $i$. If there exists a flipping point within the ball with radius $\Delta$ in identity matrix $I$, the current query is identified as sensitive. So that, it meets a condition as follow:
$\exists  \Delta _{i} \in \Delta \cdot I, f\left ( x_{q}\pm \Delta _{i} \right )\neq f\left ( x_{q} \right )$.
Then, the defender will return obfuscated response $y_{q}$ by using the boundary randomized response algorithm $BRR\left ( \cdot  \right )$ controlled by privacy budget $\epsilon $, that is: $A\left ( y_{q} \right )= \left\{\begin{matrix}
y_{q}, &w.p.  &\frac{1}{2}+\frac{\sqrt{e^{2\epsilon }-1}}{2+2e^{\epsilon }} \\ 
1-y_{q}, &w.p.  & \frac{1}{2}-\frac{\sqrt{e^{2\epsilon }-1}}{2+2e^{\epsilon }}
\end{matrix}\right.$. However, this approach will downgrade performance of the cloud-based model hosted by the cloud server.

\subsubsection{Detect by observing the query}

Apart from reducing the information returned to the attacker, a second direction is to record requests from the users, which is more realistic than output perturbation since it not impairs the utility of the cloud-based model. Kesarwani proposed Extraction Warning \cite{kesarwani2018model} to detect if an extraction attack exists and provide extraction status warnings. It requests the model owner to provide an extraction threshold $t$ and raises an alarm whenever the extraction status exceeds $t$. To measure the knowledge gained by the adversary, \cite{kesarwani2018model} introduces two methods: total information gain and coverage of the input feature space explored by the aggregated requests. The former trains and updates a local proxy model for each user to estimate the information gain with respect to a given validation set, but it is computationally expensive. The latter maintains compact query summaries and computes the feature space covered by queries relative to the class boundaries induced by the source model. 


Forgotten Siblings \cite{quiring2018forgotten} applied closeness-to-the-boundary (a concept from digital watermarking) to detect the extraction attack against decision tree. Since the adversary usually uses the queries around the decision boundary, the defender can identify malicious sequences by studying the closeness of queries to class boundaries. To be specific, firstly, it defines the security margins alongside the original decision tree boundary using the statistical distribution of the training data. Every submitted query will be recorded whether it is within the margin or not. Subsequently, the average ration $\varphi$ between queries inside and outside the margin for all leaves will be calculated. If the query ratio $\varphi$ exceeds the threshold $\tau = 0.3$, the current query will be identified as a malicious query.

However, the above schemes only work on the cloud-based models with linearly separated prediction classes (e.g., decision trees) but unavailable for the complex models like DNNs. Even worse, they ignore that a benign client may also explore large areas of the input spaces, thus raising a false alarm rate.


Then PRADA \cite{juuti2019prada}, a more generic technique, is proposed. It can be applied to detect the attacks against any cloud-based ML models. It is based on the truth that the distances between queries used by the attacker are usually artificially controlled, thus will highly deviate from a normal (Gaussian) distribution. After giving a detection threshold $\delta $, it needs to find a domain-specific distance metric $dist\left ( \right )$ to compute distances between queries. To be specific, it keeps track of the minimum distance $d_{min}\left ( x_{i_{}^{}\textrm{}} \right )$ between a new input sample $x_{i}$ and all previous samples in the same class $c$ to model the distribution of queries. And it uses the \emph{Shapiro-Wilk test statistic} $W$ to quantify if the distribution of current queries fits a normal distribution. An attack is considered to occur if $W$ is below the threshold $\delta $. However, the shortcoming of such defense is obvious: it is invalid when an adversary complements the dummy queries to fit a normal distribution.


==> modelsteal/preliminaries.tex <==
\section{Preliminaries}



\subsection{Face Recognition}

%{\color{black}Face recognition \cite{shivanna2024biometric} is a biometric technology that identifies an individual based on unique facial characteristics.} It involves comparing the features of a face in an image to those in a database of known faces to find a match. Face recognition models typically extract features (e.g., facial geometry, texture, and color) and use these features to generate a compact representation of a face, known as face embedding. Such an embedding will then be compared to embeddings of known faces to perform face recognition. 

%There are several different types of face recognition (FR) models, including convolutional neural network (CNN)-based models, DeepFace-based models, and FaceNet-based models. Each type of model has its own strengths and weaknesses. In general, deep learning-based models such as CNNs and FaceNets have achieved state-of-the-art performance on benchmark datasets and are widely used in real-world applications.

%The accuracy of face recognition models will be affected by various factors, including lighting conditions, facial expressions, and age. To improve accuracy, many real-world FR systems use multiple algorithms and combine their results to achieve a final decision. Recently, face recognition technology has been used in various applications, including security systems, mobile device authentication, and social media tagging. However, it has also raised privacy concerns, and some governments have imposed regulations on its use to protect user privacy.

Face recognition is a biometric technology that identifies individuals by analyzing unique facial features. It compares the facial characteristics in an image against a database of known faces to find a match. Typically, face recognition models extract features such as facial geometry, texture, and color, and transform them into a compact representation called a face embedding. These embeddings are then compared to embeddings in the database to recognize or verify an individual’s identity.

Several types of face recognition models are widely employed in real-world applications, including convolutional neural network (CNN)-based models, DeepFace-based models, and FaceNet-based models. Each model type offers distinct advantages in terms of accuracy, speed, and robustness. Generally, deep learning-based models such as CNNs and FaceNets have set new benchmarks for facial recognition performance and are frequently utilized in cloud-based services for tasks such as identity verification, access control, and facial authentication.

The accuracy of facial recognition systems can be affected by factors such as lighting conditions, facial expressions, and aging. To address these challenges, many cloud-based facial recognition systems integrate multiple algorithms to optimize accuracy. These systems are now being used in diverse applications, from security and surveillance to mobile device authentication and cloud-based services like photo organization. However, the widespread use of facial recognition raises significant privacy concerns, prompting regulatory bodies to impose guidelines and restrictions to protect user privacy in cloud computing environments.


\iffalse
\subsection{Online Social Networks}

{\color{black}Online social networks (OSNs) are websites or mobile applications that enable individuals to connect with each other, share content, and engage in virtual communities based on common interests or relationships.} These networks allow users to create a personal profile, upload photos and videos, share updates, and follow or add friends with other users. In the real world, popular OSNs include Facebook, Twitter, Instagram, LinkedIn, and TikTok. They play a significant role in people's lives nowadays.%allowing them to connect with friends and family, meet new people, and stay informed on current events. %However, the use of OSNs is not without challenges and controversies. In recent years, OSN also raises concerns about data privacy.  
%However, with the rise of OSNs, there has been a growing concern about the collection, use, and protection of personal information and data shared on these networks.

However, the collection and use of personal information on OSNs also raise privacy concerns. In particular, there are concerns about the security of personal information and its potential utilization for malicious purposes, such as identity theft, cyberstalking, and cyberbullying. There are also concerns about the potential for personal information to be sold or shared with third parties, such as attackers, advertisers, and commercial companies, without the consent of the users.

{\color{black}To address these concerns, various laws and regulations have been enacted to protect the privacy of personal information and data shared on OSNs \cite{fu2021robust,huang2021unlearnable}.} For example, the General Data Protection Regulation (GDPR) in Europe and the California Consumer Privacy Act (CCPA) in the United States formulate privacy regulations to protect personal information and data shared on OSNs. Despite these efforts, facial privacy protection on OSNs remains a complex and evolving issue, and users must remain vigilant in protecting their facial privacy. An effective way is to pre-process these facial photos through state-of-the-art facial protection techniques before publishing them on online social networks.

%In addition to these regulations, OSNs themselves have also implemented privacy measures to protect user data. These measures include encrypted communications, secure storage of personal information, and the implementation of privacy settings that allow users to control how their personal information is used and shared.

%Despite these efforts, data privacy on OSNs remains a complex and evolving issue, and users must remain vigilant in protecting their personal information and data. %This includes being mindful of the information they share on these networks, using privacy settings, and being aware of the terms of service and privacy policies of the OSNs they use.
%Online Social Networks (OSNs) are web-based platforms or mobile applications that allow people to connect and interact with each other, build and participate in online communities, and share information and media. These networks are designed to facilitate communication, collaboration, and information sharing among users, who can create a personal profile, connect with other users, join groups and communities, and share content such as text, images, videos, and links.

%OSNs have revolutionized the way people communicate and interact with each other. They provide users with a convenient and easy way to stay connected with friends, family, and acquaintances, as well as to expand their social network by connecting with new people who share common interests and hobbies. They also offer a platform for users to express their thoughts, opinions, and interests and to access and consume news, information, and entertainment content.

%However, the use of OSNs is not without challenges and controversies. Issues such as privacy, cyberbullying, misinformation, and the impact of social media on mental health and well-being have received growing attention in recent years. Despite these challenges, OSNs continue to be popular and widely used, with billions of people relying on them for social connection, communication, and information.



\subsection{Cloud-Based Facial Recognition Systems}
Cloud-based facial recognition systems rely on the computational power and storage capacity of cloud platforms to process and analyze large volumes of facial images. These systems enable real-time facial recognition by offloading data from user devices to cloud servers, where facial recognition models are trained and deployed at scale. The ability to store and analyze massive datasets makes cloud platforms ideal for training deep learning models used in facial recognition.

However, the integration of facial recognition technology in cloud services introduces new privacy challenges. Sensitive facial data is often transmitted and stored across distributed cloud infrastructures, exposing it to potential security breaches, unauthorized access, and exploitation. The scalability of cloud services, while advantageous for processing large datasets, can also result in the loss of control over how facial data is managed and shared across different regions and organizations.

To address these concerns, various techniques have been proposed to protect facial data in cloud environments, including encryption methods, differential privacy, and adversarial perturbations. These techniques aim to prevent unauthorized access and misuse of facial data while maintaining the utility of facial recognition systems in cloud applications.
\fi


\subsection{Cloud-Based Services and Facial Data Processing}
Cloud-based services provide vast storage and processing capabilities for handling sensitive user data, including facial images. These services are increasingly used for applications like identity verification, remote authentication, and user profile management. Cloud platforms offer scalable solutions, allowing enterprises to process facial data in real-time and across distributed regions, making them integral to modern biometric systems.

However, this convenience comes with significant privacy risks. Cloud platforms typically handle facial images for various purposes, including training facial recognition models and enabling user authentication. Given the sensitivity of facial data, unauthorized access to these images can lead to privacy breaches, identity theft, or other malicious activities, such as deepfake creation. Moreover, since cloud services often span multiple geographic locations, it is challenging for users to maintain control over how and where their facial data is stored and processed.

To address these concerns, researchers have proposed various privacy-preserving methods for facial images in cloud environments. These methods aim to protect user privacy without compromising the utility of the data in cloud-based applications. Two main categories of protection techniques are frequently explored: image obfuscation-based methods and adversarial perturbation-based methods. These methods ensure that facial images remain secure, even when processed by cloud-based face recognition systems.



==> name.tex <==
 
\section{Attacks and Defenses approaches}
In this section, we present a thorough investigation on the existing approaches of the model extraction attacks and defenses on the cloud-based models. We first classify them according to their theoretical background, then briefly describe their technical implementation details.

\subsection{Attacks Approaches}
According to the purposes of the attacker, we classify the state-of-the-art attack schemes into two categories: model attributes extraction and model functionality extraction.
\subsubsection{Model Attributes Extraction}
Nowadays, most of the extraction attack focus on attributes stealing (i.e., parameters \cite{tramer2016stealing}, hyperparameters \cite{wang2018stealing}, architecture \cite{duddu2018stealing}, and decision boundary \cite{juuti2019prada}) which are tightly related to the intellectual property rights of the cloud-based models.


Tramer et al. proposed StealML \cite{tramer2016stealing} that works on various popular cloud-based models such as logistic regression, SVM, decision tree, and shallow neural networks. It can efficiently steal the internal parameters of a black-box ML model from its prediction outputs with confidence scores. Firstly, the attacker uses a set of crafted or publicly available samples to obtain corresponding outputs $f\left (x \right )$ by querying the cloud-based model multiple times. Furthermore, he uses the input-output pairs $\left (x, f\left (x \right )\right )$ to construct a set of equations. Though solving the equations of parameters, the adversary can infer extract model parameters. Such attack is conceptually simple, but it needs to know the model family. Moreover, it only applies to simple models with small amounts of parameters and is ineffective for DNN models, which makes it a limited algorithm.


Apart from parameters, hyperparameters inside the cloud-based ML models are also of significant importance and commercial value. Wang et al. proposed StealHyperparameter \cite{wang2018stealing} to deal with the hyperparameters extraction challenges. It is based on the observation that ML algorithms determine model parameters via minimizing the objective function, and the \emph{gradient} of the objective function at the learnt model parameters is close to 0. Hence, the adversary can compute the gradient of the objective function at the model parameters and set it to 0 to obtain a system of linear equations about the hyperparameters. But, because the number of equations is generally larger than the number of unknown variables, this linear system is usually overdetermined (i.e., the number of model parameters is larger than the hyperparameters). Therefore, the authors leveraged the \emph{linear least square method} \cite{montgomery2012introduction} to estimate the hyperparameters. 


To infer the architecture of a Neural Network, Duddu et al. proposed StealNN \cite{duddu2018stealing} using the techniques of timing side channels. It is based on the truth that the total execution time of the neural network depends on the depth of the network. Besides, it assumes the adversary knows the victim's hardware and can possess the same device aiming to build timing profiles of different neural networks. Specifically, the attacker first uses iterative membership inference \cite{salem2018ml} to reconstruct its training dataset $D_{T}$, and queries the targeted model to calculate the total execution time. Then he trains a regressor on $D_{A}$ = $ \left \{ \left (T_{1},K_{1} \right ),\cdots, \left (T_{N},K_{N} \right ) \right \}$, i.e., the variation of execution time $ \left (T \right ) $ with neural network depth $\left(k\right )$. Finally, the attacker can infer the depth (the number of layers) of the DNN using the pre-trained regressor and the total execution time.




Recently, Juuti et al. \cite{juuti2019prada} presented a novel iterative model extraction strategy that includes many duplication rounds, namely PRADA. Each round consists of three phases: queries the cloud-based model $F$, trains substitute model $F'$ on the obtained labels $F(x)$, and crafts new synthetic samples based on Jacobian-Based Data Augmentation (JBDA) using the updated $F'$. Especially to deserve to be mentioned, different from other extraction methods above, one of the attack success metrics of such scheme is the transferability of the \emph{adversarial sample}, which considers extracting the decision boundary of the targeted black-box model.



\subsubsection{Model Functionality Extraction.}
Apart from the attributes extraction, another attack goal is only to construct a substitute model that can compete with the targeted cloud-based model at the same task, i.e., functionality attacks.

Shi et al. proposed StealClassifier \cite{shi2017steal} to extract the functionality of a Naive Bayes and SVM text classification classifier in the context of text classification. In this method, the authors leveraged DNN architecture to approximate the functionality of the above basic machine learning models. And they showed that the reverse is impractical, i.e., using SVM or Naive Bayes models to extract the functionality of DNN architectures.

To steal the functionality of more complex architecture, i.e., DNN models, KnockoffNets \cite{orekondy2019knockoff} is proposed. The overall phases include three parts: substitute model architecture selected, transfer dataset construct, and train the substitute model. Since the architecture of the cloud-based model is unknown to the attacker, selecting the same architecture is not a trivial thing. Fortunately, the existing theory is proved that a proper complexed architecture is enough for extracting the functionality of the common DNN model \cite{papernot2017practical,orekondy2019knockoff} even not in the same series (e.g., VGG-16 extract ResNet-10). As for the transfer dataset (i.e., image-prediction pairs) construct, the authors queried a very large benchmark datasets (e.g., ILSVRC, OpenImages) to the cloud-based model to obtain the labels. To query more efficiently, this method leverages \emph{reinforcement learning} strategies to select the best samples to query. Finally, the attacker can obtain a knockoff model after training on the transfer dataset using the selected architecture. Although it is proved effective to replicate a mature commercial API, it requires access to large sets of natural samples, which is not comparable to the synthetic samples using in \cite{juuti2019prada,papernot2017practical}.



\subsection{Defenses Approaches}

In this part, we introduce two state-of-the-art countermeasures against model extraction attacks: defending by output perturbation (i,e., injects a targeted perturbation to the model predictions) and detecting by observing the query (i.e., monitors user-server streams and generates a warning if detecting malicious behavior).
 
\subsubsection{Defence by output perturbations}

Lee \emph{et al.} proposed Deceptive Perturbations \cite{lee2019defending}, which perturbs the softmax activation function (i.e., produces the output probability) to make the attacker away from targeted parameters. Specifically, it alters original response to $\hat{y}^{i}$ in $j$-th dimension with a sum-to-one normalizer $\alpha ^{i}$: $\hat{y}^{i}_{j}= \alpha ^{i}\left ( y^{i} _{j}-r\left ( y^{i} _{j} \right )\right )$, $\hat{y}^{i}_{k}\geq \hat{y}^{i}_{j}$ for $j= 1,...,K$, where $r\left ( y^{i} _{j} \right )$ is a perturbation function called Reverse Sigmoid \cite{lee2019defending}. However, such remedy maintains the accuracy of top-1 label leading to some extraction attacks (i.e., work while discard prediction probabilities) are still effective \cite{orekondy2019knockoff,juuti2019prada}.


Based on the problem above, Orekondy \emph{et al.} proposed Prediction Poisoning \cite{orekondy2019prediction}. It is the first utility-constrained defense framework to satisfy both privacy and utility objective via introducing targeted perturbations to predictions,
that is: $\tilde{y} = \left ( 1-\alpha  \right )y+\alpha y^{*}$. 
The poisoning probability distribution $y^{*}$ satisfies the objective of mistraining the substitute model though maximizing the angular deviation between the gradient signals of poisoned posteriors and that of the original model. While $\alpha$ is a tunable parameter selected to meet accuracy-preserving utility objective $dist\left ( y,\tilde{y} \right )\leq \epsilon $, where $\epsilon$ is perturbation magnitude. The defender can trade off the utility and the security by varying $\alpha$. However, such a method requires multiple gradient computations, which results in calculation costs and inference delays increasing by orders of magnitude.


Another countermeasure is to use differential privacy to perturb the output, named BDPL \cite{zheng2019bdpl}. It appends a boundary differential private layer to perturb query response working around the decision boundary. Specifically, first it identifies whether a query $x_{q}$ is sensitive by checking corner points with projected interval $\Delta _{i}$ to $x_{q}$ on all dimension $i$. If there exists a flipping point within the ball with radius $\Delta$ in identity matrix $I$, the current query is identified as sensitive. So that, it meets a condition as follow:
$\exists  \Delta _{i} \in \Delta \cdot I, f\left ( x_{q}\pm \Delta _{i} \right )\neq f\left ( x_{q} \right )$.
Then, the defender will return obfuscated response $y_{q}$ by using the boundary randomized response algorithm $BRR\left ( \cdot  \right )$ controlled by privacy budget $\epsilon $, that is: $A\left ( y_{q} \right )= \left\{\begin{matrix}
y_{q}, &w.p.  &\frac{1}{2}+\frac{\sqrt{e^{2\epsilon }-1}}{2+2e^{\epsilon }} \\ 
1-y_{q}, &w.p.  & \frac{1}{2}-\frac{\sqrt{e^{2\epsilon }-1}}{2+2e^{\epsilon }}
\end{matrix}\right.$. However, this approach will downgrade performance of the cloud-based model hosted by the cloud server.

\subsubsection{Detect by observing the query}

Apart from reducing the information returned to the attacker, a second direction is to record requests from the users, which is more realistic than output perturbation since it not impairs the utility of the cloud-based model. Kesarwani proposed Extraction Warning \cite{kesarwani2018model} to detect if an extraction attack exists and provide extraction status warnings. It requests the model owner to provide an extraction threshold $t$ and raises an alarm whenever the extraction status exceeds $t$. To measure the knowledge gained by the adversary, \cite{kesarwani2018model} introduces two methods: total information gain and coverage of the input feature space explored by the aggregated requests. The former trains and updates a local proxy model for each user to estimate the information gain with respect to a given validation set, but it is computationally expensive. The latter maintains compact query summaries and computes the feature space covered by queries relative to the class boundaries induced by the source model. 


Forgotten Siblings \cite{quiring2018forgotten} applied closeness-to-the-boundary (a concept from digital watermarking) to detect the extraction attack against decision tree. Since the adversary usually uses the queries around the decision boundary, the defender can identify malicious sequences by studying the closeness of queries to class boundaries. To be specific, firstly, it defines the security margins alongside the original decision tree boundary using the statistical distribution of the training data. Every submitted query will be recorded whether it is within the margin or not. Subsequently, the average ration $\varphi$ between queries inside and outside the margin for all leaves will be calculated. If the query ratio $\varphi$ exceeds the threshold $\tau = 0.3$, the current query will be identified as a malicious query.

However, the above schemes only work on the cloud-based models with linearly separated prediction classes (e.g., decision trees) but unavailable for the complex models like DNNs. Even worse, they ignore that a benign client may also explore large areas of the input spaces, thus raising a false alarm rate.


Then PRADA \cite{juuti2019prada}, a more generic technique, is proposed. It can be applied to detect the attacks against any cloud-based ML models. It is based on the truth that the distances between queries used by the attacker are usually artificially controlled, thus will highly deviate from a normal (Gaussian) distribution. After giving a detection threshold $\delta $, it needs to find a domain-specific distance metric $dist\left ( \right )$ to compute distances between queries. To be specific, it keeps track of the minimum distance $d_{min}\left ( x_{i_{}^{}\textrm{}} \right )$ between a new input sample $x_{i}$ and all previous samples in the same class $c$ to model the distribution of queries. And it uses the \emph{Shapiro-Wilk test statistic} $W$ to quantify if the distribution of current queries fits a normal distribution. An attack is considered to occur if $W$ is below the threshold $\delta $. However, the shortcoming of such defense is obvious: it is invalid when an adversary complements the dummy queries to fit a normal distribution.

